Detection of the significant impact of source clustering on higher-order statistics with DES Year 3 weak gravitational lensing data

We demonstrate and measure the impact of source galaxy clustering on higher-order summary statistics of weak gravitational lensing data. By comparing simulated data with galaxies that either trace or do not trace the underlying density field, we show this effect can exceed measurement uncertainties for common higher-order statistics for certain analysis choices. Source clustering effects are larger at small scales and for statistics applied to combinations of low and high redshift samples, and diminish at high redshift. We evaluate the impact on different weak lensing observables, finding that third moments and wavelet phase harmonics are more affected than peak count statistics. Using Dark Energy Survey Year 3 data we construct null tests for the source-clustering-free case, finding a $p$-value of $p=4\times10^{-3}$ (2.6 $\sigma$) using third-order map moments and $p=3\times10^{-11}$ (6.5 $\sigma$) using wavelet phase harmonics. The impact of source clustering on cosmological inference can be either be included in the model or minimized through \textit{ad-hoc} procedures (e.g. scale cuts). We verify that the procedures adopted in existing DES Y3 cosmological analyses (using map moments and peaks) were sufficient to render this effect negligible. Failing to account for source clustering can significantly impact cosmological inference from higher-order gravitational lensing statistics, e.g. higher-order N-point functions, wavelet-moment observables (including phase harmonics and scattering transforms), and deep learning or field level summary statistics of weak lensing maps. We provide recipes both to minimise the impact of source clustering and to incorporate source clustering effects into forward-modelled mock data.

==> _.tex <==
@article{y3-BAOkp,
        author = {{DES Collaboration} and others},
        title = "{Dark Energy Survey Year 3 Results: BAO measurement}",
        year = "2020",
        journal = "To be submitted to ",
        }
        
@article{y3-baomocks,
        author = {{Ferraro}, I. and others},
        title = "{Dark Energy Survey Year 3 Results: Simulated Galaxy catalogues for BAO analysis}",
        year = "2020",
        journal = "To be submitted to MNRAS",
        }
        
@article{y3-baosample,
        author = {{Carnero Rosell}, A. and others},
        title = "{Dark Energy Survey Year 3 Results: Galaxy Sample for BAO Measurement}",
        year = "2020",
        journal = "To be submitted to MNRAS",
        }

@article{y3-gold,
       author = {{Sevilla-Noarbe}, I. and {Bechtol}, K. and {Carrasco Kind}, M. and {Carnero Rosell}, A. and {Becker}, M.~R. and {Drlica-Wagner}, A. and {Gruendl}, R.~A. and {Rykoff}, E.~S. and {Sheldon}, E. and {Yanny}, B. and {Alarcon}, A. and {Allam}, S. and {Amon}, A. and {Benoit-L{\'e}vy}, A. and {Bernstein}, G.~M. and {Bertin}, E. and {Burke}, D.~L. and {Carretero}, J. and {Choi}, A. and {Diehl}, H.~T. and {Everett}, S. and {Flaugher}, B. and {Gaztanaga}, E. and {Gschwend}, J. and {Harrison}, I. and {Hartley}, W.~G. and {Hoyle}, B. and {Jarvis}, M. and {Johnson}, M.~D. and {Kessler}, R. and {Kron}, R. and {Kuropatkin}, N. and {Leistedt}, B. and {Li}, T.~S. and {Menanteau}, F. and {Morganson}, E. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Pieres}, A. and {Pond}, C. and {Rodriguez-Monroy}, M. and {Smith}, J. Allyn and {Stringer}, K.~M. and {Troxel}, M.~A. and {Tucker}, D.~L. and {de Vicente}, J. and {Wester}, W. and {Zhang}, Y. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Annis}, J. and {Avila}, S. and {Bhargava}, S. and {Bridle}, S.~L. and {Brooks}, D. and {Brout}, D. and {Castander}, F.~J. and {Cawthon}, R. and {Chang}, C. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Davis}, T.~M. and {Desai}, S. and {Dietrich}, J.~P. and {Doel}, P. and {Eckert}, K. and {Evrard}, A.~E. and {Ferrero}, I. and {Fosalba}, P. and {Garc{\'\i}a-Bellido}, J. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gruen}, D. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Huff}, E.~M. and {Huterer}, D. and {James}, D.~J. and {Jeltema}, T. and {Kuehn}, K. and {Lahav}, O. and {Lidman}, C. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Neilsen}, E. and {Plazas}, A.~A. and {Romer}, A.~K. and {Roodman}, A. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Smith}, M. and {Suchyta}, E. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Wechsler}, R.~H. and {Weller}, J. and {Wilkinson}, R.~D. and {DES Collaboration}},
        title = "{Dark Energy Survey Year 3 Results: Photometric Data Set for Cosmology}",
      journal = {\apjs},
     keywords = {Surveys, Catalogs, Observational cosmology, 1671, 205, 1146, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = jun,
       volume = {254},
       number = {2},
          eid = {24},
        pages = {24},
          doi = {10.3847/1538-4365/abeb66},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021ApJS..254...24S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-balrog,
       author = {{Everett}, S. and {Yanny}, B. and {Kuropatkin}, N. and {Huff}, E.~M. and {Zhang}, Y. and {Myles}, J. and {Masegian}, A. and {Elvin-Poole}, J. and {Allam}, S. and {Bernstein}, G.~M. and {Sevilla-Noarbe}, I. and {Splettstoesser}, M. and {Sheldon}, E. and {Jarvis}, M. and {Amon}, A. and {Harrison}, I. and {Choi}, A. and {Hartley}, W.~G. and {Alarcon}, A. and {S{\'a}nchez}, C. and {Gruen}, D. and {Eckert}, K. and {Prat}, J. and {Tabbutt}, M. and {Busti}, V. and {Becker}, M.~R. and {MacCrann}, N. and {Diehl}, H.~T. and {Tucker}, D.~L. and {Bertin}, E. and {Jeltema}, T. and {Drlica-Wagner}, A. and {Gruendl}, R.~A. and {Bechtol}, K. and {Carnero Rosell}, A. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Annis}, J. and {Bacon}, D. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Conselice}, C. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {DeRose}, J. and {Desai}, S. and {Eifler}, T.~F. and {Evrard}, A.~E. and {Ferrero}, I. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Huterer}, D. and {James}, D.~J. and {Kent}, S. and {Krause}, E. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Muir}, J. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Romer}, A.~K. and {Roodman}, A. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {To}, C. and {Troxel}, M.~A. and {Varga}, T.~N. and {Weller}, J. and {Wilkinson}, R.~D.},
        title = "{Dark Energy Survey Year 3 Results: Measuring the Survey Transfer Function with Balrog}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.12825},
        pages = {arXiv:2012.12825},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201212825E},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-deepfields,
       author = {{Hartley}, W.~G. and {Choi}, A. and {Amon}, A. and {Gruendl}, R.~A. and {Sheldon}, E. and {Harrison}, I. and {Bernstein}, G.~M. and {Sevilla-Noarbe}, I. and {Yanny}, B. and {Eckert}, K. and {Diehl}, H.~T. and {Alarcon}, A. and {Banerji}, M. and {Bechtol}, K. and {Buchs}, R. and {Cantu}, S. and {Conselice}, C. and {Cordero}, J. and {Davis}, C. and {Davis}, T.~M. and {Dodelson}, S. and {Drlica-Wagner}, A. and {Everett}, S. and {Fert{\'e}}, A. and {Gruen}, D. and {Honscheid}, K. and {Jarvis}, M. and {Johnson}, M.~D. and {Kokron}, N. and {MacCrann}, N. and {Myles}, J. and {Pace}, A.~B. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Pereira}, M.~E.~S. and {Plazas}, A.~A. and {Prat}, J. and {Rodriguez-Monroy}, M. and {Rykoff}, E.~S. and {Samuroff}, S. and {S{\'a}nchez}, C. and {Secco}, L.~F. and {Tarsitano}, F. and {Tong}, A. and {Troxel}, M.~A. and {Vasquez}, Z. and {Wang}, K. and {Zhou}, C. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {De Vicente}, J. and {DeRose}, J. and {Desai}, S. and {Dietrich}, J.~P. and {Eifler}, T.~F. and {Elvin-Poole}, J. and {Ferrero}, I. and {Flaugher}, B. and {Fosalba}, P. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Huterer}, D. and {James}, D.~J. and {Kent}, S. and {Krause}, E. and {Kuehn}, K. and {Kuropatkin}, N. and {Lahav}, O. and {Lin}, H. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Neilsen}, E. and {Ogando}, R.~L.~C. and {Pandey}, S. and {Romer}, A.~K. and {Roodman}, A. and {Sako}, M. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Walker}, A.~R. and {Wester}, W. and {Wilkinson}, R.~D. and {Zuntz}, J.},
        title = "{Dark Energy Survey Year 3 Results: Deep Field Optical + Near-Infrared Images and Catalogue}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.12824},
        pages = {arXiv:2012.12824},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201212824H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{y3-shapecatalog,
       author = {{Gatti}, M. and {Sheldon}, E. and {Amon}, A. and {Becker}, M. and {Troxel}, M. and {Choi}, A. and {Doux}, C. and {MacCrann}, N. and {Navarro-Alsina}, A. and {Harrison}, I. and {Gruen}, D. and {Bernstein}, G. and {Jarvis}, M. and {Secco}, L.~F. and {Fert{\'e}}, A. and {Shin}, T. and {McCullough}, J. and {Rollins}, R.~P. and {Chen}, R. and {Chang}, C. and {Pandey}, S. and {Tutusaus}, I. and {Prat}, J. and {Elvin-Poole}, J. and {Sanchez}, C. and {Plazas}, A.~A. and {Roodman}, A. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {Davis}, T.~M. and {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Dietrich}, J.~P. and {Doel}, P. and {Drlica-Wagner}, A. and {Eckert}, K. and {Everett}, S. and {Ferrero}, I. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hartley}, W.~G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {Huff}, E.~M. and {Huterer}, D. and {Jain}, B. and {James}, D.~J. and {Jeltema}, T. and {Krause}, E. and {Kron}, R. and {Kuropatkin}, N. and {Lima}, M. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Miquel}, R. and {Morgan}, R. and {Myles}, J. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Rykoff}, E.~S. and {Samuroff}, S. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Tucker}, D.~L. and {Varga}, T.~N. and {Wechsler}, R.~H. and {Weller}, J. and {Wester}, W. and {Wilkinson}, R.~D.},
        title = "{Dark energy survey year 3 results: weak lensing shape catalogue}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, methods: data analysis, techniques: image processing, catalogues, surveys, cosmology: observations, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = jul,
       volume = {504},
       number = {3},
        pages = {4312-4336},
          doi = {10.1093/mnras/stab918},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.504.4312G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{y3-piff,
       author = {{Jarvis}, M. and {Bernstein}, G.~M. and {Amon}, A. and {Davis}, C. and {L{\'e}get}, P.~F. and {Bechtol}, K. and {Harrison}, I. and {Gatti}, M. and {Roodman}, A. and {Chang}, C. and {Chen}, R. and {Choi}, A. and {Desai}, S. and {Drlica-Wagner}, A. and {Gruen}, D. and {Gruendl}, R.~A. and {Hernandez}, A. and {MacCrann}, N. and {Meyers}, J. and {Navarro-Alsina}, A. and {Pandey}, S. and {Plazas}, A.~A. and {Secco}, L.~F. and {Sheldon}, E. and {Troxel}, M.~A. and {Vorperian}, S. and {Wei}, K. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Avila}, S. and {Bhargava}, S. and {Bridle}, S.~L. and {Brooks}, D. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Costanzi}, M. and {da Costa}, L.~N. and {De Vicente}, J. and {Diehl}, H.~T. and {Doel}, P. and {Everett}, S. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {James}, D.~J. and {Kent}, S. and {Kuehn}, K. and {Kuropatkin}, N. and {Lahav}, O. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Ogando}, R.~L.~C. and {Paz-Chinch{\'o}n}, F. and {Rykoff}, E.~S. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Varga}, T.~N. and {Walker}, A.~R. and {Wester}, W. and {Wilkinson}, R.~D. and {DES Collaboration}},
        title = "{Dark Energy Survey year 3 results: point spread function modelling}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, techniques: image processing, catalogues, surveys, software: data analysis, cosmology: observations, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = feb,
       volume = {501},
       number = {1},
        pages = {1282-1299},
          doi = {10.1093/mnras/staa3679},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.501.1282J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-imagesims,
       author = {{MacCrann}, N. and {Becker}, M.~R. and {McCullough}, J. and {Amon}, A. and {Gruen}, D. and {Jarvis}, M. and {Choi}, A. and {Troxel}, M.~A. and {Sheldon}, E. and {Yanny}, B. and {Herner}, K. and {Dodelson}, S. and {Zuntz}, J. and {Eckert}, K. and {Rollins}, R.~P. and {Varga}, T.~N. and {Bernstein}, G.~M. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Sevilla-Noarbe}, I. and {Pieres}, A. and {Bridle}, S.~L. and {Myles}, J. and {Alarcon}, A. and {Everett}, S. and {S{\'a}nchez}, C. and {Huff}, E.~M. and {Tarsitano}, F. and {Gatti}, M. and {Secco}, L.~F. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Bacon}, D. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Costanzi}, M. and {Crocce}, M. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Dietrich}, J.~P. and {Doel}, P. and {Eifler}, T.~F. and {Ferrero}, I. and {Fert{\'e}}, A. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {James}, D.~J. and {Lahav}, O. and {Lima}, M. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Muir}, J. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Roodman}, A. and {Samuroff}, S. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Wilkinson}, R.~D.},
        title = "{DES Y3 results: Blending shear and redshift biases in image simulations}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.08567},
        pages = {arXiv:2012.08567},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201208567M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{y3-sompz,
author = {{Myles}, J. and {Alarcon}, A. and {Amon}, A. and {S{\'a}nchez}, C. and {Everett}, S. and {DeRose}, J. and {McCullough}, J. and {Gruen}, D. and {Bernstein}, G.~M. and {Troxel}, M.~A. and {Dodelson}, S. and {Campos}, A. and {MacCrann}, N. and {Yin}, B. and {Raveri}, M. and {Amara}, A. and {Becker}, M.~R. and {Choi}, A. and {Cordero}, J. and {Eckert}, K. and {Gatti}, M. and {Giannini}, G. and {Gschwend}, J. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Huff}, E.~M. and {Kuropatkin}, N. and {Lin}, H. and {Masters}, D. and {Miquel}, R. and {Prat}, J. and {Roodman}, A. and {Rykoff}, E.~S. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Wechsler}, R.~H. and {Yanny}, B. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Bridle}, S.~L. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Desai}, S. and {Diehl}, H.~T. and {Eifler}, T.~F. and {Elvin-Poole}, J. and {Evrard}, A.~E. and {Ferrero}, I. and {Fert{\'e}}, A. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Giannantonio}, T. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {Huterer}, D. and {James}, D.~J. and {Krause}, E. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Mohr}, J.~J. and {Morgan}, R. and {Muir}, J. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Samuroff}, S. and {Sanchez}, E. and {Scarpine}, V. and {Secco}, L.~F. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Weller}, J. and {Wester}, W.},
        title = "{Dark Energy Survey Year 3 results: redshift calibration of the weak lensing source galaxies}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, galaxies: distances and redshifts, dark energy, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = aug,
       volume = {505},
       number = {3},
        pages = {4249-4277},
          doi = {10.1093/mnras/stab1515},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.505.4249M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-sourcewz,
       author = {{Gatti}, M. and {Giannini}, G. and {Bernstein}, G.~M. and {Alarcon}, A. and {Myles}, J. and {Amon}, A. and {Cawthon}, R. and {Troxel}, M. and {DeRose}, J. and {Everett}, S. and {Ross}, A.~J. and {Rykoff}, E.~S. and {Elvin-Poole}, J. and {Cordero}, J. and {Harrison}, I. and {Sanchez}, C. and {Prat}, J. and {Gruen}, D. and {Lin}, H. and {Crocce}, M. and {Rozo}, E. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Choi}, A. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Dawson}, K. and {Desai}, S. and {Diehl}, H.~T. and {Eckert}, K. and {Eifler}, T.~F. and {Evrard}, A.~E. and {Ferrero}, I. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garcia-Bellido}, J. and {Gaztanaga}, E. and {Giannantonio}, T. and {Gruendl}, R.~A. and {Gschwend}, J. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {Huterer}, D. and {James}, D.~J. and {Kuehn}, K. and {Kuropatkin}, N. and {Lahav}, O. and {Lima}, M. and {MacCrann}, N. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinchon}, F. and {Percival}, W.~J. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Roodman}, A. and {Rossi}, G. and {Samuroff}, S. and {Sanchez}, E. and {Scarpine}, V. and {Secco}, L.~F. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Weller}, J. and {Wilkinson}, R.~D.},
        title = "{Dark Energy Survey Year 3 Results: Clustering Redshifts -- Calibration of the Weak Lensing Source Redshift Distributions with redMaGiC and BOSS/eBOSS}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.08569},
        pages = {arXiv:2012.08569},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201208569G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{y3-lenswz,
       author = {{Cawthon}, R. and {Elvin-Poole}, J. and {Porredon}, A. and {Crocce}, M. and {Giannini}, G. and {Gatti}, M. and {Ross}, A.~J. and {Rykoff}, E.~S. and {Carnero Rosell}, A. and {DeRose}, J. and {Lee}, S. and {Rodriguez-Monroy}, M. and {Amon}, A. and {Bechtol}, K. and {De Vicente}, J. and {Gruen}, D. and {Morgan}, R. and {Sanchez}, E. and {Sanchez}, J. and {Sevilla-Noarbe}, I. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Choi}, A. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Dawson}, K. and {Desai}, S. and {Diehl}, H.~T. and {Eckert}, K. and {Everett}, S. and {Ferrero}, I. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Huterer}, D. and {James}, D.~J. and {Kim}, A.~G. and {Kneib}, J. -P. and {Kuehn}, K. and {Kuropatkin}, N. and {Lahav}, O. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Muir}, J. and {Myles}, J. and {Palmese}, A. and {Pandey}, S. and {Paz-Chinch{\'o}n}, F. and {Percival}, W.~J. and {Plazas}, A.~A. and {Roodman}, A. and {Rossi}, G. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {To}, C. and {Troxel}, M.~A. and {Wilkinson}, R.~D. and {the DES Collaboration}},
        title = "{Dark Energy Survey Year 3 Results: Calibration of Lens Sample Redshift Distributions using Clustering Redshifts with BOSS/eBOSS}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.12826},
        pages = {arXiv:2012.12826},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201212826C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{y3-sompzbuzzard,
       author = {{Buchs}, R. and {Davis}, C. and {Gruen}, D. and {DeRose}, J. and
         {Alarcon}, A. and {Bernstein}, G.~M. and {S{\'a}nchez}, C. and
         {Myles}, J. and {Roodman}, A. and {Allen}, S. and {Amon}, A. and
         {Choi}, A. and {Masters}, D.~C. and {Miquel}, R. and {Troxel}, M.~A. and
         {Wechsler}, R.~H. and {Abbott}, T.~M.~C. and {Annis}, J. and
         {Avila}, S. and {Bechtol}, K. and {Bridle}, S.~L. and {Brooks}, D. and
         {Buckley-Geer}, E. and {Burke}, D.~L. and {Carnero Rosell}, A. and
         {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and
         {Cawthon}, R. and {D'Andrea}, C.~B. and {da Costa}, L.~N. and
         {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Doel}, P. and
         {Drlica-Wagner}, A. and {Eifler}, T.~F. and {Evrard}, A.~E. and
         {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and
         {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gruendl}, R.~A. and
         {Gschwend}, J. and {Gutierrez}, G. and {Hartley}, W.~G. and
         {Hollowood}, D.~L. and {Honscheid}, K. and {James}, D.~J. and
         {Kuehn}, K. and {Kuropatkin}, N. and {Lima}, M. and {Lin}, H. and
         {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and
         {Melchior}, P. and {Menanteau}, F. and {Ogando}, R.~L.~C. and
         {Plazas}, A.~A. and {Rykoff}, E.~S. and {Sanchez}, E. and
         {Scarpine}, V. and {Serrano}, S. and {Sevilla-Noarbe}, I. and
         {Smith}, M. and {Soares-Santos}, M. and {Sobreira}, F. and
         {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and
         {Vikram}, V. and {DES Collaboration}},
        title = "{Phenotypic redshifts with self-organizing maps: A novel method to characterize redshift distributions of source galaxies for weak lensing}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, galaxies: distances and redshifts, dark energy, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2019,
        month = oct,
       volume = {489},
       number = {1},
        pages = {820-841},
          doi = {10.1093/mnras/stz2162},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489..820B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-hyperrank,
        author = {{Cordero}, Juan P. and {Harrison}, Ian and {Rollins}, Richard P. and {Bernstein}, G.~M. and {Bridle}, S.~L. and {Alarcon}, A. and {Alves}, O. and {Amon}, A. and {Andrade-Oliveira}, F. and {Camacho}, H. and {Campos}, A. and {Choi}, A. and {DeRose}, J. and {Dodelson}, S. and {Eckert}, K. and {Eifler}, T.~F. and {Everett}, S. and {Fang}, X. and {Friedrich}, O. and {Gruen}, D. and {Gruendl}, R.~A. and {Hartley}, W.~G. and {Huff}, E.~M. and {Krause}, E. and {Kuropatkin}, N. and {MacCrann}, N. and {McCullough}, J. and {Myles}, J. and {Pandey}, S. and {Raveri}, M. and {Rosenfeld}, R. and {Rykoff}, E.~S. and {S{\'a}nchez}, C. and {S{\'a}nchez}, J. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Troxel}, M. and {Wechsler}, R. and {Yanny}, B. and {Yin}, B. and {Zhang}, Y. and {Aguena}, M. and {Allam}, S. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Cawthon}, R. and {Costanzi}, M. and {da Costa}, L. and {da Silva Pereira}, M.~E. and {De Vicente}, J. and {Diehl}, H.~T. and {Dietrich}, J. and {Doel}, P. and {Elvin-Poole}, J. and {Ferrero}, I. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garcia-Bellido}, J. and {Gerdes}, D. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {James}, D. and {Kuehn}, K. and {Lahav}, O. and {Maia}, M.~A.~G. and {March}, M. and {Menanteau}, F. and {Miquel}, R. and {Morgan}, R. and {Muir}, J. and {Palmese}, A. and {Paz-Chinchon}, F. and {Pieres}, A. and {Plazas Malag{\'o}n}, A. and {S{\'a}nchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N.},
        title = "{Dark Energy Survey Year 3 results: Marginalisation over redshift distribution uncertainties using ranking of discrete realisations}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = sep,
          eid = {arXiv:2109.09636},
        pages = {arXiv:2109.09636},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210909636C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-shearratio,
        author = {{S{\'a}nchez}, C. and {Prat}, J. and {Zacharegkas}, G. and {Pandey}, S. and {Baxter}, E. and {Bernstein}, G.~M. and {Blazek}, J. and {Cawthon}, R. and {Chang}, C. and {Krause}, E. and {Lemos}, P. and {Park}, Y. and {Raveri}, M. and {Sanchez}, J. and {Troxel}, M.~A. and {Amon}, A. and {Fang}, X. and {Friedrich}, O. and {Gruen}, D. and {Porredon}, A. and {Secco}, L.~F. and {Samuroff}, S. and {Alarcon}, A. and {Alves}, O. and {Andrade-Oliveira}, F. and {Bechtol}, K. and {Becker}, M.~R. and {Camacho}, H. and {Campos}, A. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Chen}, R. and {Choi}, A. and {Crocce}, M. and {Davis}, C. and {De Vicente}, J. and {DeRose}, J. and {Di Valentino}, E. and {Diehl}, H.~T. and {Dodelson}, S. and {Doux}, C. and {Drlica-Wagner}, A. and {Eckert}, K. and {Eifler}, T.~F. and {Elsner}, F. and {Elvin-Poole}, J. and {Everett}, S. and {Fert{\'e}}, A. and {Fosalba}, P. and {Gatti}, M. and {Giannini}, G. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Herner}, K. and {Huff}, E.~M. and {Huterer}, D. and {Jarvis}, M. and {Jain}, B. and {Kuropatkin}, N. and {Leget}, P. -F. and {MacCrann}, N. and {McCullough}, J. and {Muir}, J. and {Myles}, J. and {Navarro-Alsina}, A. and {Rollins}, R.~P. and {Roodman}, A. and {Rosenfeld}, R. and {Rykoff}, E.~S. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Shin}, T. and {Troja}, A. and {Tutusaus}, I. and {Varga}, T.~N. and {Wechsler}, R.~H. and {Yanny}, B. and {Yin}, B. and {Zhang}, Y. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Buckley-Geer}, E. and {Burke}, D.~L. and {Carretero}, J. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Desai}, S. and {Dietrich}, J.~P. and {Doel}, P. and {Evrard}, A.~E. and {Ferrero}, I. and {Flaugher}, B. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {James}, D.~J. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Petravick}, D. and {Pieres}, A. and {Plazas Malag{\'o}n}, A.~A. and {Rodriguez-Monroy}, M. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C.},
        title = "{Dark Energy Survey Year 3 Results: Exploiting small-scale information with lensing shear ratios}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.13542},
        pages = {arXiv:2105.13542},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210513542S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-simvalidation,
        author = {{DeRose}, J. and others},
        title = "{Dark Energy Survey Year 3 Results: Validating $3\times2$-point Modeling and Analysis Choices using Cosmological Simulations}",
        year = "2021",
        journal = "To be submitted to ",
        }

@article{y3-samplers,
        author = {{Surname}, A. and others},
        title = "{Dark Energy Survey Year 3 Results: }",
        year = "2020",
        journal = "To be submitted to ",
        }

@article{y3-tensions,
       author = {{Lemos}, P. and {Raveri}, M. and {Campos}, A. and {Park}, Y. and {Chang}, C. and {Weaverdyck}, N. and {Huterer}, D. and {Liddle}, A.~R. and {Blazek}, J. and {Cawthon}, R. and {Choi}, A. and {DeRose}, J. and {Dodelson}, S. and {Doux}, C. and {Gatti}, M. and {Gruen}, D. and {Harrison}, I. and {Krause}, E. and {Lahav}, O. and {MacCrann}, N. and {Muir}, J. and {Prat}, J. and {Rau}, M.~M. and {Rollins}, R.~P. and {Samuroff}, S. and {Zuntz}, J. and {Hartley}, W.~G. and {Hoyle}, B. and {Sevilla-Noarbe}, I. and {Troxel}, M.~A. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Avila}, S. and {Bacon}, D. and {Bernstein}, G.~M. and {Bertin}, E. and {Brooks}, D. and {Burke}, D.~L. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Carretero}, J. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Doel}, P. and {Eckert}, K. and {Eifler}, T.~F. and {Elvin-Poole}, J. and {Everett}, S. and {Evrard}, A.~E. and {Ferrero}, I. and {Fert{\'e}}, A. and {Flaugher}, B. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Huff}, E.~M. and {James}, D.~J. and {Jarvis}, M. and {Lima}, M. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Myles}, J. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Pandey}, S. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Roodman}, A. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Secco}, L.~F. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Weller}, J. and {Wester}, W.},
        title = "{Assessing tension metrics with Dark Energy Survey and Planck data}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.09554},
        pages = {arXiv:2012.09554},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201209554L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-inttensions,
       author = {{Doux}, C. and {Baxter}, E. and {Lemos}, P. and {Chang}, C. and {Alarcon}, A. and {Amon}, A. and {Campos}, A. and {Choi}, A. and {Gatti}, M. and {Gruen}, D. and {Jarvis}, M. and {MacCrann}, N. and {Park}, Y. and {Prat}, J. and {Rau}, M.~M. and {Raveri}, M. and {Samuroff}, S. and {DeRose}, J. and {Hartley}, W.~G. and {Hoyle}, B. and {Troxel}, M.~A. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carrasco Kind}, M. and {Carretero}, J. and {Cawthon}, R. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {Desai}, S. and {Diehl}, H.~T. and {Dietrich}, J.~P. and {Doel}, P. and {Everett}, S. and {Ferrero}, I. and {Fosalba}, P. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Huff}, E.~M. and {Huterer}, D. and {Jain}, B. and {James}, D.~J. and {Krause}, E. and {Kuehn}, K. and {Kuropatkin}, N. and {Lahav}, O. and {Lidman}, C. and {Lima}, M. and {Maia}, M.~A.~G. and {Menanteau}, F. and {Miquel}, R. and {Morgan}, R. and {Muir}, J. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {To}, C. and {Tucker}, D.~L. and {Varga}, T.~N. and {Weller}, J. and {Wilkinson}, R.~D.},
        title = "{Dark energy survey internal consistency tests of the joint cosmological probes analysis with posterior predictive distributions}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, methods: statistical, dark energy, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2021,
        month = may,
       volume = {503},
       number = {2},
        pages = {2688-2705},
          doi = {10.1093/mnras/stab526},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.503.2688D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-covariances,
       author = {{Friedrich}, O. and {Andrade-Oliveira}, F. and {Camacho}, H. and {Alves}, O. and {Rosenfeld}, R. and {Sanchez}, J. and {Fang}, X. and {Eifler}, T.~F. and {Krause}, E. and {Chang}, C. and {Omori}, Y. and {Amon}, A. and {Baxter}, E. and {Elvin-Poole}, J. and {Huterer}, D. and {Porredon}, A. and {Prat}, J. and {Terra}, V. and {Troja}, A. and {Alarcon}, A. and {Bechtol}, K. and {Bernstein}, G.~M. and {Buchs}, R. and {Campos}, A. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Cawthon}, R. and {Choi}, A. and {Cordero}, J. and {Crocce}, M. and {Davis}, C. and {DeRose}, J. and {Diehl}, H.~T. and {Dodelson}, S. and {Doux}, C. and {Drlica-Wagner}, A. and {Elsner}, F. and {Everett}, S. and {Fosalba}, P. and {Gatti}, M. and {Giannini}, G. and {Gruen}, D. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Jain}, B. and {Jarvis}, M. and {MacCrann}, N. and {McCullough}, J. and {Muir}, J. and {Myles}, J. and {Pandey}, S. and {Raveri}, M. and {Roodman}, A. and {Rodriguez-Monroy}, M. and {Rykoff}, E.~S. and {Samuroff}, S. and {S{\'a}nchez}, C. and {Secco}, L.~F. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Troxel}, M.~A. and {Weaverdyck}, N. and {Yanny}, B. and {Aguena}, M. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carretero}, J. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Evrard}, A.~E. and {Ferrero}, I. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {James}, D.~J. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Maia}, M.~A.~G. and {Menanteau}, F. and {Miquel}, R. and {Morgan}, R. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Soares-Santos}, M. and {Smith}, M. and {Suchyta}, E. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Varga}, T.~N. and {Weller}, J. and {Wilkinson}, R.~D.},
        title = "{Dark Energy Survey Year 3 Results: Covariance Modelling and its Impact on Parameter Estimation and Quality of Fit}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2020,
        month = dec,
          eid = {arXiv:2012.08568},
        pages = {arXiv:2012.08568},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201208568F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{y3-blinding,
       author = {{Muir}, J. and {Bernstein}, G.~M. and {Huterer}, D. and {Elsner}, F. and
         {Krause}, E. and {Roodman}, A. and {Allam}, S. and {Annis}, J. and
         {Avila}, S. and {Bechtol}, K. and {Bertin}, E. and {Brooks}, D. and
         {Buckley-Geer}, E. and {Burke}, D.~L. and {Carnero Rosell}, A. and
         {Carrasco Kind}, M. and {Carretero}, J. and {Cawthon}, R. and
         {Costanzi}, M. and {da Costa}, L.~N. and {De Vicente}, J. and
         {Desai}, S. and {Dietrich}, J.~P. and {Doel}, P. and {Eifler}, T.~F. and
         {Everett}, S. and {Fosalba}, P. and {Frieman}, J. and
         {Garc{\'\i}a-Bellido}, J. and {Gerdes}, D.~W. and {Gruen}, D. and
         {Gruendl}, R.~A. and {Gschwend}, J. and {Hartley}, W.~G. and
         {Hollowood}, D.~L. and {James}, D.~J. and {Jarvis}, M. and {Kuehn}, K. and
         {Kuropatkin}, N. and {Lahav}, O. and {March}, M. and {Marshall}, J.~L. and
         {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Ogand
        o}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and
         {Plazas}, A.~A. and {Romer}, A.~K. and {Sanchez}, E. and
         {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and
         {Sevilla-Noarbe}, I. and {Smith}, M. and {Suchyta}, E. and {Tarle}, G. and
         {Thomas}, D. and {Troxel}, M.~A. and {Walker}, A.~R. and {Weller}, J. and
         {Wester}, W. and {Zuntz}, J. and {DES Collaboration}},
        title = "{Blinding multiprobe cosmological experiments}",
      journal = {\mnras},
     keywords = {methods: data analysis, methods: numerical, methods: statistical, cosmology: observations; large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2020,
        month = apr,
       volume = {494},
       number = {3},
        pages = {4454-4470},
          doi = {10.1093/mnras/staa965},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.494.4454M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-generalmethods,
        author = {{Krause}, E. and others},
        title = "{Dark Energy Survey Year 3 Results: Multi-probe modeling validation}",
        year = "2021",
        journal = "To be submitted to MNRAS",
        }

@article{y3-massmapping,
        author = {{Jeffrey}, N. and {Gatti}, M. and {Chang}, C. and {Whiteway}, L. and {Demirbozan}, U. and {Kovacs}, A. and {Pollina}, G. and {Bacon}, D. and {Hamaus}, N. and {Kacprzak}, T. and {Lahav}, O. and {Lanusse}, F. and {Mawdsley}, B. and {Nadathur}, S. and {Starck}, J.~L. and {Vielzeuf}, P. and {Zeurcher}, D. and {Alarcon}, A. and {Amon}, A. and {Bechtol}, K. and {Bernstein}, G.~M. and {Campos}, A. and {Rosell}, A. Carnero and {Kind}, M. Carrasco and {Cawthon}, R. and {Chen}, R. and {Choi}, A. and {Cordero}, J. and {Davis}, C. and {DeRose}, J. and {Doux}, C. and {Drlica-Wagner}, A. and {Eckert}, K. and {Elsner}, F. and {Elvin-Poole}, J. and {Everett}, S. and {Fert{\'e}}, A. and {Giannini}, G. and {Gruen}, D. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Herner}, K. and {Huff}, E.~M. and {Huterer}, D. and {Kuropatkin}, N. and {Jarvis}, M. and {Leget}, P.~F. and {MacCrann}, N. and {McCullough}, J. and {Muir}, J. and {Myles}, J. and {Navarro-Alsina}, A. and {Pandey}, S. and {Prat}, J. and {Raveri}, M. and {Rollins}, R.~P. and {Ross}, A.~J. and {Rykoff}, E.~S. and {S{\'a}nchez}, C. and {Secco}, L.~F. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Shin}, T. and {Troxel}, M.~A. and {Tutusaus}, I. and {Varga}, T.~N. and {Yanny}, B. and {Yin}, B. and {Zhang}, Y. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Andrade-Oliveira}, F. and {Becker}, M.~R. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Burke}, D.~L. and {Carretero}, J. and {Castander}, F.~J. and {Conselice}, C. and {Costanzi}, M. and {Crocce}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Dietrich}, J.~P. and {Doel}, P. and {Ferrero}, I. and {Flaugher}, B. and {Fosalba}, P. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Hoyle}, B. and {Jain}, B. and {James}, D.~J. and {Lima}, M. and {Maia}, M.~A.~G. and {March}, M. and {Marshall}, J.~L. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Roodman}, A. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Weller}, J. and {DES Collaboration}},
        title = "{Dark Energy Survey Year 3 results: Curved-sky weak lensing mass map reconstruction}",
      journal = {\mnras},
     keywords = {gravitational lensing: weak, methods: statistical, large-scale structure of Universe, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = aug,
       volume = {505},
       number = {3},
        pages = {4626-4645},
          doi = {10.1093/mnras/stab1495},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021MNRAS.505.4626J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-galaxyclustering,
        author = {{Rodr\'iguez-Monroy}, M. and others},
        title = "{Dark Energy Survey Year 3 Results: Galaxy clustering and systematics treatment for lens galaxy samples}",
        year = "2021",
        journal = "To be submitted to MNRAS",
        }

@article{y3-gglensing,
        author = {{Prat}, J. and others},
        title = "{Dark Energy Survey Year 3 Results: Accurate measurement and modeling of galaxy-galaxy lensing}",
        year = "2021",
        journal = "To be submitted to MNRAS",
        }

@article{y3-cosmicshear1,
        author = {{Amon}, A. and {Gruen}, D. and {Troxel}, M.~A. and {MacCrann}, N. and {Dodelson}, S. and {Choi}, A. and {Doux}, C. and {Secco}, L.~F. and {Samuroff}, S. and {Krause}, E. and {Cordero}, J. and {Myles}, J. and {DeRose}, J. and {Wechsler}, R.~H. and {Gatti}, M. and {Navarro-Alsina}, A. and {Bernstein}, G.~M. and {Jain}, B. and {Blazek}, J. and {Alarcon}, A. and {Fert{\'e}}, A. and {Raveri}, M. and {Lemos}, P. and {Campos}, A. and {Prat}, J. and {S{\'a}nchez}, C. and {Jarvis}, M. and {Alves}, O. and {Andrade-Oliveira}, F. and {Baxter}, E. and {Bechtol}, K. and {Becker}, M.~R. and {Bridle}, S.~L. and {Camacho}, H. and {Campos}, A. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Cawthon}, R. and {Chang}, C. and {Chen}, R. and {Chintalapati}, P. and {Crocce}, M. and {Davis}, C. and {Diehl}, H.~T. and {Drlica-Wagner}, A. and {Eckert}, K. and {Eifler}, T.~F. and {Elvin-Poole}, J. and {Everett}, S. and {Fang}, X. and {Fosalba}, P. and {Friedrich}, O. and {Giannini}, G. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Herner}, K. and {Huang}, H. and {Huff}, E.~M. and {Huterer}, D. and {Kuropatkin}, N. and {Leget}, P. -F. and {Liddle}, A.~R. and {McCullough}, J. and {Muir}, J. and {Pandey}, S. and {Park}, Y. and {Porredon}, A. and {Refregier}, A. and {Rollins}, R.~P. and {Roodman}, A. and {Rosenfeld}, R. and {Ross}, A.~J. and {Rykoff}, E.~S. and {Sanchez}, J. and {Sevilla-Noarbe}, I. and {Sheldon}, E. and {Shin}, T. and {Troja}, A. and {Tutusaus}, I. and {Varga}, T.~N. and {Weaverdyck}, N. and {Yanny}, B. and {Yin}, B. and {Zhang}, Y. and {Zuntz}, J. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Brooks}, D. and {Buckley-Geer}, E. and {Burke}, D.~L. and {Carretero}, J. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Dietrich}, J.~P. and {Doel}, P. and {Ferrero}, I. and {Flaugher}, B. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {James}, D.~J. and {Kron}, R. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Petravick}, D. and {Pieres}, A. and {Plazas Malag{\'o}n}, A.~A. and {Romer}, A.~K. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Tarle}, G. and {Thomas}, D. and {To}, C. and {Weller}, J.},
        title = "{Dark Energy Survey Year 3 Results: Cosmology from Cosmic Shear and Robustness to Data Calibration}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.13543},
        pages = {arXiv:2105.13543},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210513543A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@article{y3-cosmicshear2,
       author = {{Secco}, L.~F. and {Samuroff}, S. and {Krause}, E. and {Jain}, B. and {Blazek}, J. and {Raveri}, M. and {Campos}, A. and {Amon}, A. and {Chen}, A. and {Doux}, C. and {Choi}, A. and {Gruen}, D. and {Bernstein}, G.~M. and {Chang}, C. and {DeRose}, J. and {Myles}, J. and {Fert{\'e}}, A. and {Lemos}, P. and {Huterer}, D. and {Prat}, J. and {Troxel}, M.~A. and {MacCrann}, N. and {Liddle}, A.~R. and {Kacprzak}, T. and {Fang}, X. and {S{\'a}nchez}, C. and {Pandey}, S. and {Dodelson}, S. and {Chintalapati}, P. and {Hoffmann}, K. and {Alarcon}, A. and {Alves}, O. and {Andrade-Oliveira}, F. and {Baxter}, E.~J. and {Bechtol}, K. and {Becker}, M.~R. and {Brandao-Souza}, A. and {Camacho}, H. and {Carnero Rosell}, A. and {Carrasco Kind}, M. and {Cawthon}, R. and {Cordero}, J.~P. and {Crocce}, M. and {Davis}, C. and {Di Valentino}, E. and {Drlica-Wagner}, A. and {Eckert}, K. and {Eifler}, T.~F. and {Elidaiana}, M. and {Elsner}, F. and {Elvin-Poole}, J. and {Everett}, S. and {Fosalba}, P. and {Friedrich}, O. and {Gatti}, M. and {Giannini}, G. and {Gruendl}, R.~A. and {Harrison}, I. and {Hartley}, W.~G. and {Herner}, K. and {Huang}, H. and {Huff}, E.~M. and {Jarvis}, M. and {Jeffrey}, N. and {Kuropatkin}, N. and {Leget}, P. -F. and {Muir}, J. and {Mccullough}, J. and {Navarro Alsina}, A. and {Omori}, Y. and {Park}, Y. and {Porredon}, A. and {Rollins}, R. and {Roodman}, A. and {Rosenfeld}, R. and {Ross}, A.~J. and {Rykoff}, E.~S. and {Sanchez}, J. and {Sevilla-Noarbe}, I. and {Sheldon}, E.~S. and {Shin}, T. and {Tutusaus}, I. and {Varga}, T.~N. and {Weaverdyck}, N. and {Wechsler}, R.~H. and {Yanny}, B. and {Yin}, B. and {Zhang}, Y. and {Zuntz}, J. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Annis}, J. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Bridle}, S.~L. and {Brooks}, D. and {Buckley-Geer}, E. and {Burke}, D.~L. and {Carretero}, J. and {Costanzi}, M. and {da Costa}, L.~N. and {De Vicente}, J. and {Diehl}, H.~T. and {Dietrich}, J.~P. and {Doel}, P. and {Ferrero}, I. and {Flaugher}, B. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gschwend}, J. and {Gutierrez}, G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {James}, D.~J. and {Jeltema}, T. and {Kuehn}, K. and {Lahav}, O. and {Lima}, M. and {Lin}, H. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Martini}, P. and {Melchior}, P. and {Menanteau}, F. and {Miquel}, R. and {Mohr}, J.~J. and {Morgan}, R. and {Ogando}, R.~L.~C. and {Palmese}, A. and {Paz-Chinch{\'o}n}, F. and {Petravick}, D. and {Pieres}, A. and {Plazas Malag{\'o}n}, A.~A. and {Rodriguez-Monroy}, M. and {Romer}, A.~K. and {Sanchez}, E. and {Scarpine}, V. and {Schubnell}, M. and {Scolnic}, D. and {Serrano}, S. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {Thomas}, D. and {To}, C.},
        title = "{Dark Energy Survey Year 3 Results: Cosmology from Cosmic Shear and Robustness to Modeling Uncertainty}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.13544},
        pages = {arXiv:2105.13544},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210513544S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{y3-2x2ptbiasmodelling,
        author = {{Pandey}, S. and others},
        title = "{Dark Energy Survey Year 3 Results: Constraints on cosmological parameters and galaxy bias models from galaxy clustering and galaxy-galaxy lensing}",
        year = "2021",
        journal = "To be submitted to MNRAS",
        }

@article{y3-2x2ptmagnification,
        author = {{Elvin-Poole}, J. and others},
        title = "{Dark Energy Survey Year 3 Results: Measurement, modelling and cosmological impact of magnification in galaxy clustering and galaxy-galaxy lensing}",
        year = "2021",
        journal = "To be submitted to MNRAS",
        }

@article{y3-2x2maglimforecast,
	author = {{Porredon}, A. and {Crocce}, M. and {Fosalba}, P. and {Elvin-Poole}, J. and {Carnero Rosell}, A. and {Cawthon}, R. and {Eifler}, T.~F. and {Fang}, X. and {Ferrero}, I. and {Krause}, E. and {MacCrann}, N. and {Weaverdyck}, N. and {Abbott}, T.~M.~C. and {Aguena}, M. and {Allam}, S. and {Amon}, A. and {Avila}, S. and {Bacon}, D. and {Bertin}, E. and {Bhargava}, S. and {Bridle}, S.~L. and {Brooks}, D. and {Carrasco Kind}, M. and {Carretero}, J. and {Castander}, F.~J. and {Choi}, A. and {Costanzi}, M. and {da Costa}, L.~N. and {Pereira}, M.~E.~S. and {De Vicente}, J. and {Desai}, S. and {Diehl}, H.~T. and {Doel}, P. and {Drlica-Wagner}, A. and {Eckert}, K. and {Fert{\'e}}, A. and {Flaugher}, B. and {Frieman}, J. and {Garc{\'\i}a-Bellido}, J. and {Gaztanaga}, E. and {Gerdes}, D.~W. and {Giannantonio}, T. and {Gruen}, D. and {Gruendl}, R.~A. and {Gschwend}, J. and {Gutierrez}, G. and {Hartley}, W.~G. and {Hinton}, S.~R. and {Hollowood}, D.~L. and {Honscheid}, K. and {Hoyle}, B. and {James}, D.~J. and {Jarvis}, M. and {Kuehn}, K. and {Kuropatkin}, N. and {Maia}, M.~A.~G. and {Marshall}, J.~L. and {Menanteau}, F. and {Miquel}, R. and {Morgan}, R. and {Palmese}, A. and {Pandey}, S. and {Paz-Chinch{\'o}n}, F. and {Plazas}, A.~A. and {Rodriguez-Monroy}, M. and {Roodman}, A. and {Samuroff}, S. and {Sanchez}, E. and {Scarpine}, V. and {Serrano}, S. and {Sevilla-Noarbe}, I. and {Smith}, M. and {Soares-Santos}, M. and {Suchyta}, E. and {Swanson}, M.~E.~C. and {Tarle}, G. and {To}, C. and {Varga}, T.~N. and {Weller}, J. and {Wilkinson}, R.~D.},
	title = "{Dark Energy Survey Year 3 Results: Optimizing the Lens Sample in Combined Galaxy Clustering and Galaxy-Galaxy Lensing Analysis}",
	 journal = {\prd},
	keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
	year = 2021,
	month = feb,
        volume = {103},
	number = {4},
	eid = {043503},
	pages = {043503},
	doi = {10.1103/PhysRevD.103.043503},
	primaryClass = {astro-ph.CO},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2020arXiv201103411P},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{y3-2x2ptaltlensresults,
        author = {{Porredon}, A. and others},
        title = "{Dark Energy Survey Year 3 Results: Cosmological Constraints from Galaxy Clustering and Galaxy-Galaxy Lensing using an Optimized Lens Sample}",
        year = "in prep.",
        journal = "To be submitted to PRD",
        }

@article{y3-3x2ptkp,
         author = {{DES Collaboration}},
        title = "{Dark Energy Survey Year 3 Results: Cosmological Constraints from Galaxy Clustering and Weak Lensing}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2021,
        month = may,
          eid = {arXiv:2105.13549},
        pages = {arXiv:2105.13549},
 primaryClass = {astro-ph.CO},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210513549D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



==> convergence_t.tex <==
\section{Convergence test}
Probably worth showing the effect is there in different simulations (DarkGrid, my sims, Niall&Lorne's HR sims).
